Picard and Brauer groups of $K(n)$-local spectra via profinite Galois descent

Using the pro\'etale site, we construct models for the continuous actions of the Morava stabiliser group on Morava E-theory, its $\infty$-category of $K(n)$-local modules, and its Picard spectrum. For the two sheaves of spectra, we evaluate the resulting descent spectral sequences: these can be thought of as homotopy fixed point spectral sequences for the profinite Galois extension $L_{K(n)} \mathbb S \to E_n$. We show that the descent spectral sequence for the Morava E-theory sheaf is the $K(n)$-local $E_n$-Adams spectral sequence. The spectral sequence for the sheaf of Picard spectra is closely related to one recently defined by Heard; our formalism allows us to compare many differentials with those in the $K(n)$-local $E_n$-Adams spectral sequence, and isolate the exotic Picard elements in the $0$-stem. In particular, we show how this recovers the computation due to Hopkins, Mahowald and Sadofsky of the group $\mathrm{Pic}_1$ at all primes. We also use these methods to bound the Brauer group of $K(n)$-local spectra, and compute this bound at height one.

==> scrap/Tools.tex <==
\subsubsection{Computational tools}
In \cref{sec:brauer descent} that the $(-1)$-stem of the descent spectral sequence for the Picard sheaf gives an upper bound on the size of the relative Brauer group $\Br(\bm 1_\K \mid \E)$, and we have used this to compute the height one Brauer groups at odd primes. To attack the computation at $p = 2$ we would like some quantitative refinements of this result. Firstly, we develop an obstruction theory for existence and uniqueness of lifts of Azumaya algebras over $\E$ to $\bm 1_\K$; this is analogous to \cite[§6.5 and Theorem~7.17]{gl}. We would also like to give a spectral sequence using Postnikov invariants of the spectrum $\pic \E$ and group cohomology to compute Postnikov invariants of the sheaf $\pic(\mathcal E)$ (thought of as a spectrum with continuous $\G$-action); again, this is inspired by the methods of \cite{gl}.

Namely, we consider the map $\Br(\bm 1_\K \mid \E) \to \pi_0 \Tot \Brr_0'(\E^{\bullet})$; this admits an obstruction theory in the sense of \cite{bousfield-obstruction}.

\begin{thm}
Suppose $A \in \pi_0 \Tot \Brr_0'(\E^\bullet)$. The obstructions to existence and uniqueness of a lift $A' \in \Brr(\bm 1_\K)$ are computed as follows:
\begin{enumerate}
    \item if $A_0$ is the image of $A$ in $\Br(\E)$ and $A' \in \Br(\bm 1_\K)$ is such that $A' \otimes \E \simeq A_0$, then the obstruction to uniqueness of $A'$
\end{enumerate}
\end{thm}






\subsubsection*{Equivariant mapping spectra}
In order to compute the upper bound for $\Br(\bm 1_\K)$ arising from \cref{lem:relative Brauer spectrum is a subspace of lim BPiccun(R' bullet)} we need a better understanding of the descent spectral sequence for $\Picc(\mathcal E)$; namely, we need to compute the $(-1)$-stem. In order to compute differentials to the left of the $y$-axis, it will be useful to compute a small number $k$-invariants of $\pic(\mathcal E)$ relative to the t-structure on $\Sh[\mathcal Sp]{\proet \G}$. We will give a general formalism for doing so, similar to the results of \cite[§??]{gl}. Namely, our objective is to prove that for suitable $X,Y \in \Sh[\mathcal Sp]{\proet \G}$ there is a spectral sequence of the form
    \[ H^{t-s}_{\mathrm{cont}}(\G, \pi_t \Map[]{X, Y}) \implies \Map[\G]{X,Y}, \]
allowing us (at least in theory) to compute equivariant $k$-invariants from the data of non-equivariant $k$-invariants together with the group action. We will set out the necessary conditions on $X$ and $Y$, and use this to compute differentials in the $(-1)$-stem of the Picard spectral sequence at height one in \cref{sec:Brauer n=1}.

For the rest of the section, $G$ is an arbitrary profinite group.

\begin{defn}
For a site $\mathcal C$, a spectrum $k$ and $X, Y \in \Sh[\mathcal Sp_k]{\mathcal C}$, we write $\Mapsh[\mathcal C]{X,Y} = \Mapsh[]{X,Y}$ for the presheaf of mapping spaces from $X$ to $Y$: for fixed $X$, $\mapsh[\mathcal C]{X,-}$ is right-adjoint to
    \[ (-) \otimes X: \mathcal P \left(\mathcal C \right) \to \Psh[\mathcal Sp_k]{\mathcal C}. \]
In particular, 
\begin{equation} \label{eqn:Yoneda formula for sheaf mapping spaces}
    \Gamma \left(C, \Mapsh[\mathcal C]{X,Y} \right) \simeq \Map[\mathcal C]{h_C, \Mapsh[\mathcal C]{X,Y}} \simeq \Map[\mathcal C]{h_C \otimes X, Y} \simeq [???] \Map[\mathcal C_{/C}]{h_C \otimes X, h_C \otimes Y}.
\end{equation}
If $Y$ is a sheaf and $V_\bullet \to U$ is the \v Cech complex of a covering, then
\begin{align*}
    \Map[\mathcal C]{h_{V_\bullet}, \Mapsh[\mathcal C]{X,Y}} &\simeq \Map[\mathcal C]{h_{V_\bullet}, \Mapsh[\mathcal C]{X,Y}} \\
    & \simeq \Map[\mathcal C]{X, \Mapsh[\mathcal C]{L_k \Sigma^\infty_+ h_{V_\bullet},Y}} \\
    & \simeq \Map[\mathcal C]{X, \Mapsh[\mathcal C]{L_k \Sigma^\infty_+ h_U,Y}} \\
    & \simeq \Map[\mathcal C]{h_U, \Mapsh[\mathcal C]{X,Y}},
\end{align*}
so $\Mapsh[\mathcal C]{X,Y}$ is a a sheaf too; likewise, if $Y$ is a hypersheaf then so is $\Mapsh[\mathcal C]{X,Y}$.

In fact, the functor
    \[ (-) \otimes X: \Psh[\mathcal Sp_k]{\mathcal C} \to \Psh[\mathcal Sp_k]{\mathcal C} \]
itself admits a right adjoint $\mapsh[\mathcal C]{X,-}$, and $\Mapsh[\mathcal C]{X,Y} \simeq \Omega^\infty \mapsh[\mathcal C]{X,Y}$ since $Z \otimes X = L_k \Sigma^\infty_+ Z \otimes X$ for any sheaf of spaces $Z$.
\end{defn}

We are particularly interested in the case $\mathcal C = \proet G$, when we will write $\Mapsh[G]{X,Y}$ for $\Mapsh[\proet G]{X,Y}$. By taking a Postnikov tower in $\mathcal{S}h \left( \proet G \right)$, we obtain a spectral sequence
    \[ H^{t-s}(\proet G, \pi_t \Mapsh[G]{X,Y}) \implies \pi_t \Map[G]{X,Y}. \]
Our next task is to understand the $E_1$-page, under assumptions on $X$ and $Y$.

\begin{defn}
If $\mathcal C$ is complete and cocomplete, a \emph{condensed object} of $\mathcal C$ is a hypercomplete sheaf $A: \Profin \op \to \mathcal C$. We will say that the condensed topology on $A$ is \emph{discrete} if $A$ is Kan extended from $\Fin \subset \Profin$: that is, for any profinite set $T$ with presentation $T = \lim_i T_i$, we require that
    \[ \varinjlim_i A(T_i) \xrightarrow{\sim} A(T). \]
\end{defn}

\begin{ex}
If $G$ is a profinite group then $(\proet G)_{/G} \simeq \Profin$, so any $X \in \Sh[\mathcal C]{\proet G}$ has an underlying condensed object given by its restriction to any $G$-torsor.
\end{ex}

Recall the restricted Yoneda embedding $\Top \to \mathrm{Cond}(\Set)$, which is fully faithful on compactly-generated spaces. We will abuse notation to identify the profinite group $G$ with its Yoneda image. This is a group object of $\mathrm{Cond}(\Set)$, and therefore has an \inftycat{} of modules in $\mathrm{Cond}(\mathcal C)$ for any cocomplete $\mathcal C$, using the tensor $\Set \otimes \mathcal C \to \mathcal C$.

\begin{prop}
For any $G$-torsor $X$, the forgetful functor $j: \mathcal (\proet G)_{/X} \to \mathcal \mathcal \proet G$ induces an equivalence
    \[ \Shh[\mathcal C]{\proet G} \simeq \Mod_{G} \left(\mathrm{Cond}(\mathcal C) \right). \]
\end{prop}

\begin{proof}
The functor $j$ is a map of sites, and so induces an adjunction
    \[ j^*: \Shh[\mathcal C]{(\proet G)_{/X}} \simeq \mathrm{Cond}(\mathcal C) \rightleftarrows \Shh[\mathcal C]{\proet G}: j_*. \]
Our first claim is that $j_*$ is monadic, and so factors through an equivalence
\begin{equation}
    \Shh[\mathcal C]{\proet G} \simeq \Mod_{\mathbb T} \left( \mathrm{Cond}(\mathcal C) \right),
\end{equation}
where $\mathbb T$ is the monad $j_* j^*: \mathrm{Cond}(\mathcal C) \to \mathrm{Cond}(\mathcal C)$. We will deduce this from the Barr-Beck-Lurie theorem, and must therefore justify the following:
\begin{enumerate}
    \item $j_*$ is conservative. Indeed, any profinite $G$-set is covered by a free one. A map $\mathcal F \to \mathcal F'$ such that $j_* F \simeq j_* \mathcal F$ is therefore locally an equivalence, and so an equivalence.
    \item $j_*$-split simplicial objects in $\Shh[\mathcal C]{\proet G}$ admit realisations, and these are preserved by $j_*$. The first is automatic, since $\Shh[\mathcal C]{\proet G}$ has all colimits. Furthermore, $j_*$ admits a \emph{right} adjoint, given by the \emph{right} Kan extension
% https://q.uiver.app/?q=WzAsMyxbMCwwLCIoXFxwcm9ldCBHKV97L1h9Il0sWzEsMSwiXFxwcm9ldCBHIl0sWzIsMCwiXFxtYXRoY2FsIEMiXSxbMCwyLCJcXG1hdGhjYWwgRiJdLFswLDEsImoiLDJdLFsxLDIsImpeISBcXG1hdGhjYWwgRiIsMix7InN0eWxlIjp7ImJvZHkiOnsibmFtZSI6ImRhc2hlZCJ9fX1dXQ==
\[\begin{tikzcd}[ampersand replacement=\&,column sep=small]
	{(\proet G)_{/X}} \&\& {\mathcal C} \\
	\& {\proet G}
	\arrow["{\mathcal F}", from=1-1, to=1-3]
	\arrow["j"', from=1-1, to=2-2]
	\arrow[%"{j^{!} \mathcal F}"', 
        dashed, from=2-2, to=1-3]
\end{tikzcd}\]
    and so preserves all colimits.
\end{enumerate}

Next, we identify the monad $\mathbb T$; we will show it agrees with the functor $G \otimes (-) : \mathrm{Cond}(\mathcal C) \to \mathrm{Cond}(\mathcal C)$. If $\mathcal F$ is a condensed object of $\mathcal C$, then 
    
\end{proof}
























\begin{lem}
Suppose that the condensed topology on $X|_{G}$ is discrete. Suppose also that [...???]. Then 
    \[ \pi_t \Mapsh[G]{X,Y} = \Cont[G]{-, \pi_t \Map{X,Y}}. \]
As a result, the descent spectral sequence for $\Mapsh[\G]{X,Y}$ takes the form
    \[ H^{t-s}_{\mathrm{cont}}(G, \Map{X,Y}) \implies \pi_t \Map[G]{X,Y}. \]
\end{lem}

\begin{proof}
Suppose $S = G \times T$ is a free $G$-set. Using \cref{eqn:Yoneda formula for sheaf mapping spaces}, we compute
\begin{align*}
    \pi_t \Gamma(S, \Mapsh[G]{X,Y}) &\simeq \pi_t \Map[G]{X|_S, Y} \\
    & \simeq [???] \Map[(\proet G)_{/G}]{X|_{T \times G}, Y|_G} \\
    & \simeq \pi_t \Map[\Profin]{(X|_G)|_{T}, Y|_G} \\
    & \simeq \pi_t \lim_i \prod_{T_i} \Map{X(G), Y(G)} \\
\end{align*}
\end{proof}

\begin{cor}
Under the assumptions of the previous lemma, the Postnikov tower for $\mapsh[G]{X,Y}$ converges, and so its descent spectral sequence converges conditionally.
\end{cor}

\begin{proof}
The same proof as for \cref{lem:hyperdescent for presheaf extension of mathcal E} works here.
\end{proof}







